Data-driven Optimization for the Evolve-Filter-Relax regularization of convection-dominated flows

Numerical stabilization techniques are often employed in under-resolved simulations of convection-dominated flows to improve accuracy and mitigate spurious oscillations. Specifically, the evolve--filter--relax (EFR) algorithm is a framework which consists in evolving the solution, applying a filtering step to remove high-frequency noise, and relaxing through a convex combination of filtered and original solutions. The stability and accuracy of the EFR solution strongly depend on two parameters, the filter radius $\delta$ and the relaxation parameter $\chi$. Standard choices for these parameters are usually fixed in time, and related to the full order model setting, i.e., the grid size for $\delta$ and the time step for $\chi$. The key novelties with respect to the standard EFR approach are: (i) time-dependent parameters $\delta(t)$ and $\chi(t)$, and (ii) data-driven adaptive optimization of the parameters in time, considering a fully-resolved simulation as reference. In particular, we propose three different classes of optimized-EFR (Opt-EFR) strategies, aiming to optimize one or both parameters. The new Opt-EFR strategies are tested in the under-resolved simulation of a turbulent flow past a cylinder at $Re=1000$. The Opt-EFR proved to be more accurate than standard approaches by up to 99$\%$, while maintaining a similar computational time. In particular, the key new finding of our analysis is that such accuracy can be obtained only if the optimized objective function includes: (i) a global metric (as the kinetic energy), and (ii) spatial gradients' information.

==> sections/preamble_wiley.tex <==

%\usepackage[foot]{amsaddr}
\usepackage{comment}
%\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{verbatim}
\usepackage{subfig}
\usepackage{amsmath,amssymb}
\usepackage{mathtools}
\usepackage{siunitx}
\usepackage{xcolor}
%\usepackage{xcolor}
%\usepackage[top=1in, bottom=1.25in, left=1.25in, right=1.25in]{geometry}
%\usepackage{geometry}
%\usepackage[hidelinks]{hyperref}
%\usepackage{algorithm}% http://ctan.org/pkg/algorithms
%\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx
\usepackage{algpseudocode}
\usepackage{ulem}

\newcommand{\ms}[1]{{ \color{magenta}{[MS - #1]}}}
\newcommand{\ai}[1]{{ \color{teal}{[AI - #1]}}}
\newcommand{\mg}[1]{{ \color{red}{[MG - #1]}}}
\newcommand{\ti}[1]{{\color{blue}{[TI - #1]}}}
\newcommand{\graybox}[1]{\colorbox{gray!30}{\parbox{\linewidth}{#1}}}

\newcommand{\highlight}[1]{\colorbox{gray!30}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{#1}}}

\usepackage{booktabs}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\usepackage{float} 
\definecolor{mediumpurple}{rgb}{0.58, 0.0, 0.83}
\newcommand{\RA}[1]{{{\color{green!60!black}#1}}}
\newcommand{\RB}[1]{{\color{red}#1}}
\newcommand{\RALL}[1]{{\color{mediumpurple}#1}}

